Numerical study of Wigner negativity in one-dimensional steady-state resonance fluorescence

In a numerical study, we investigate the steady-state generation of nonclassical states of light from a coherently driven two-level atom in a one-dimensional waveguide. Specifically, we look for states with a negative Wigner function, since such nonclassical states are a resource for quantum information processing applications, including quantum computing. We find that a waveguide terminated by a mirror at the position of the atom can provide Wigner-negative states, while an infinite waveguide yields strictly positive Wigner functions. Moreover, our investigation reveals a connection between the purity of a quantum state and its Wigner negativity. We also analyze the effects of decoherence on the negativity of a state.

==> method/coherent_disp.tex <==


%Phase information encoded by the off-diagonal elements of the density matrix signifies quantum coherence. 


if we consider a mixture of pure states,then we can not expect in general to observe intensity fringes of maximum contrast. Certain particular mixtures of one photon states may, however, preserve the factorization property Eq. (2.109) of the correlation function and thereby preserve the coherence property. Hence we must not think of pure states as the only ones which bring about coherence


Pure states need not be coherent, and coherent states need not be pure.\cite{ballentine1998quantum}

chaotic light has g1=0

pure single photon is 1st order coherent. but it is highly nonclassical. 

can get interference fringes from a signle photon, provided it has a non-zero probability to be in two-different modes. 

Fields with vanishing mean values of  will be referred to as unphased fields. https://journals.aps.org/pr/pdf/10.1103/PhysRev.131.2766
that is glaubers paper, here is another https://journals.aps.org/pr/pdf/10.1103/PhysRev.130.2529


coherence is often defined in terms of the g2 function, ref loudon

g1 increasing with time https://www.jstor.org/stable/pdf/36623.pdf?refreqid=excelsior%3A240cfb35357e79b209269d89673342ee


\begin{enumerate}
    \item Coherent and pure \\
    coherent state $\ket\alpha$
    \item coherent but not pure\\
    multimode coherent state
    \item pure but not coherent\\
    two-mode state $\ket{1,1}$ with one photon in each mode 
    \item neither pure nor coherent\\
    blackbody radiation
\end{enumerate}

%%%%%%%%%%%%%%%%%%%
Shih: An intro to QO

thermal light is often called incoherent
thermal state is mixed

an incoherent light beam must be described as a statistical mixture of all the excitation states available for each mode excited \url{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.10.84}

incoherent fields, or the broad class off ields for which the correlation functions do not factorize, \url{https://journals.aps.org/pr/abstract/10.1103/PhysRev.131.2766}



thermal=chaotic=gaussian=incoherent=(g2=2)


at the incoherent point, the emitted field contains no phase information, and should thus be symmetric (around the origin) in phase space? No. it is centered at 0 though, because <a>=0. It is well known that a coherent state is displaced from the origin by <a>=|alpha|. But it is more general, in general the state is centered a distance <a> away from the origin. 












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The mean photon number of photons in a coherent state is 
\begin{equation}\label{n}
    \braket{n}=\braket{\adagger\hat a}=|\alpha|^2=\frac{x^2+P^2}{2}.
\end{equation}


\subsection{Coherent displacement at weak driving strength}


With driving strength $\Omega$, the number of photons sent on average per unit time is $\Omega^2$. Over a time $T$, we expect a coherent state $\ket\alpha$ with a mean number of photons 
%
\begin{equation}
\braket{n}=|\alpha|^2=\Omega^2T.
\end{equation}
%
With $P=0$ \textcolor{red}{why?} in~\eqref{n}, we have 
%
\begin{equation}\label{xpos}
    |x|=\sqrt{2T}\Omega.
\end{equation}
%
Simulations agree with this, see Fig.~\ref{coherent_refl}.

\begin{figure}[H] 
    \centering
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width=1\textwidth]{{{bilder/W_T100_Omega0.1}}}
        \caption{$x=-\sqrt{2}$}
    \end{subfigure}%
    %
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width=1\textwidth]{{{bilder/W_T200_Omega0.05}}}
        \caption{$x=-1$}
    \end{subfigure}
          \caption{Very weak driving. The line is at $x=-\sqrt{2T}\Omega$, according to~\eqref{xpos}. The center of the Wigner function is displaced as expected for a coherent state. This means that the reflected signal is coherent. }
          \label{coherent_refl}
          % data in exjobb_program/run_dir
          %N=7, 1000 trajs, 30 angles, 2000 maxlik iterations 
\end{figure}

\subsection{Stronger weak driving}
\textcolor{red}{put hats on operators?}

For stronger driving, still in the weak driving regime, The Wigner function is closer to the origin than expected for a coherent state. 
\begin{figure}[H]  
    \centering
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width=1\textwidth]{{{bilder/W_T15_Omega0.5}}}
        \caption{kkkk}
    \end{subfigure}%
    %
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width=1\textwidth]{{{bilder/W_T10_Omega0.6}}}
        \caption{kkkkkk}
    \end{subfigure}
          \caption{löklökö }
          \label{coherent_refl1}
          % data in exjobb_program/run_dir
          %N=7, 1000 trajs, 30 angles, 2000 maxlik iterations 
\end{figure}

With
%
\begin{equation}
    A=\frac{1}{\sqrt{T}}\int_0^T \dt\,\aout(t),
\end{equation}
%
we have the number operator
%
\begin{equation}
    \braket{A^\dagger A}=\frac{1}{T} \int_0^T \dt_1\int_0^T \dt_2 \braket{\aout^\dagger(t_1)\aout(t_2)}.
\end{equation}
%
Using the input-output relation~\eqref{ain_aout} and the fact that we are only looking at the reflected field, we have 
%
\begin{equation}
      \braket{\aout^\dagger(t_1)\aout(t_2)} = \gamma'\braket{\sigmaplus(t_1)\sigmaminus(t_2)}. 
\end{equation}
%
we get
%
\begin{equation}
      \braket{A^\dagger A}=\frac{\gamma'}{T} \int_0^T \dt_1\int_0^T \dt_2\braket{\sigmaplus(t_1)\sigmaminus(t_2)}
\end{equation}

....
\begin{equation}
      \braket{A^\dagger A}=\gamma'T|\steady{\braket{\sigmaminus}}|^2
\end{equation}


Combining this expression of $\braket{N}$ with Eq.~\eqref{n} gives \textcolor{red}{inconsistent notation}
\begin{equation}
    x=-\frac{\sqrt{2T}\Omega}{1+4\Omega^2}
\end{equation}


==> results/negativity.tex <==

%¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤4



